Canary Extraction in Natural Language Understanding Models

Natural Language Understanding (NLU) models can be trained on sensitive information such as phone numbers, zip-codes etc. Recent literature has focused on Model Inversion Attacks (ModIvA) that can extract training data from model parameters. In this work, we present a version of such an attack by extracting canaries inserted in NLU training data. In the attack, an adversary with open-box access to the model reconstructs the canaries contained in the model's training set. We evaluate our approach by performing text completion on canaries and demonstrate that by using the prefix (non-sensitive) tokens of the canary, we can generate the full canary. As an example, our attack is able to reconstruct a four digit code in the training dataset of the NLU model with a probability of 0.5 in its best configuration. As countermeasures, we identify several defense mechanisms that, when combined, effectively eliminate the risk of ModIvA in our experiments.

==> ethics_review.tex <==
% \pdfoutput=1
% % In particular, the hyperref package requires pdfLaTeX in order to break URLs across lines.

% \documentclass[11pt]{article}

% % Remove the "review" option to generate the final version.
% \usepackage[review]{acl}
% % \usepackage{emnlp2021}

% % Standard package includes
% \usepackage{times}
% \usepackage{latexsym}
% \renewcommand{\UrlFont}{\ttfamily\small}
% \usepackage{comment}
% \usepackage{bm}
% \usepackage{siunitx}
% \usepackage{booktabs}
% \usepackage{adjustbox}
% \usepackage{graphicx}
% \usepackage{latexsym}
% \usepackage{amsmath}
% \usepackage [english]{babel}
% \usepackage{multirow}
% \usepackage{caption}
% \usepackage{subcaption}
% %%% HELPER CODE FOR DEALING WITH EXTERNAL REFERENCES
% \usepackage{xr}
% \usepackage{hyperref}
% \makeatletter
% \newcommand*{\addFileDependency}[1]{
%   \typeout{(#1)}
%   \@addtofilelist{#1}
%   \IfFileExists{#1}{}{\typeout{No file #1.}}
% }
% \makeatother

% \newcommand*{\myexternaldocument}[1]{
%     \externaldocument{#1}
%     \addFileDependency{#1.tex}
%     \addFileDependency{#1.aux}
% }


% % For proper rendering and hyphenation of words containing Latin characters (including in bib files)
% \usepackage[T1]{fontenc}
% % For Vietnamese characters
% % \usepackage[T5]{fontenc}
% % See https://www.latex-project.org/help/documentation/encguide.pdf for other character sets

% % This assumes your files are encoded as UTF8
% \usepackage[utf8]{inputenc}

% % This is not strictly necessary, and may be commented out,
% % but it will improve the layout of the manuscript,
% % and will typically save some space.
% \usepackage{microtype}

% % If the title and author information does not fit in the area allocated, uncomment the following
% %
% %\setlength\titlebox{<dim>}
% %
% % and set <dim> to something 5cm or larger.

% % Author information can be set in various styles:
% % For several authors from the same institution:
% % \author{Author 1 \and ... \and Author n \\
% %         Address line \\ ... \\ Address line}
% % if the names do not fit well on one line use
% %         Author 1 \\ {\bf Author 2} \\ ... \\ {\bf Author n} \\
% % For authors from different institutions:
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \And  ... \And
% %         Author n \\ Address line \\ ... \\ Address line}
% % To start a seperate ``row'' of authors use \AND, as in
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \AND
% %         Author 2 \\ Address line \\ ... \\ Address line \And
% %         Author 3 \\ Address line \\ ... \\ Address line}

% \begin{document}
% Ethics Review Received:
% \textit{Recommendation: 1 - No serious ethical issues
% Ethics Review:
% Please address this reviewer's comment: the proposed attack can also be potentially misused to extract private information from public datasets and crowd-sourced data by an adversary with white-box access to the trained model.}

% We thank the ethics reviewers for their comments. We have made the following changes to the manuscript to address the same. 

% Addition of Section 6: Proposed Defenses Against ModIvA:
% Through our work we aim to warn NLU researchers of the risks associated with training on private information and help them prevent such attacks. We recognize that the defenses against Model Inversion Attacks are of equal importance to the reader as the attack itself. For this reason we have included a new section describing the defense mechanisms in more detail in the manuscript-- Section 6: Proposed Defenses Against ModIvA. This section describes how NLU practitioners can effectively protect NLU models against such attacks. 

% Changes in Section 8: Ethical Considerations:
% Model Inversion Attacks have been demonstrated on computer vision task \cite{fredrikson2015model} where the model inputs are continuous and NLU task \cite{song2020information} where the model outputs are continuous. In our work we adapted this type of attack to NLU models where both the inputs and outputs are discrete. As discussed in Section 8: Ethical Considerations, with our experiments we wish to demonstrate that most NLU models are vulnerable to such attacks. In doing so, we encourage NLU researchers to acknowledge the risk is no longer hypothetical and to address this risk when developing new models. We believe studying the vulnerabilities of such attacks is a necessary step to prevent its harm.

% % In Table 3 we have demonstrate that these defenses can be used to prevent the attack completely. 

% % We acknowledge that the attack may potentially be misused to extract private information from public datasets with white-box access to existing models. However, as detailed in Section 6, we note that if a model is trained with one of the three common modeling techniques-- dropout, early stopping or using character embeddings, the risk of such an attack may drastically reduce. 

% % We discuss the potential risks associated with our work in Section 8: Ethical Considerations. We emphasize on the intended objectives of this study and recommend mechanisms to safeguard NLU models against misuse. We strongly emphasize that NLU practitioners should be more attentive while working on datasets with private information. We also discuss the use of scientific artifacts in our work. 

% \bibliographystyle{acl_natbib}
% \bibliography{custom}

% \end{document}
